Geometric ergodicity of the bouncy particle sampler

The Bouncy Particle Sampler (BPS) is a Monte Carlo Markov Chain algorithm to sample from a target density known up to a multiplicative constant. This method is based on a kinetic piecewise deterministic Markov process for which the target measure is invariant. This paper deals with theoretical properties of BPS. First, we establish geometric ergodicity of the associated semi-group under weaker conditions than in [10] both on the target distribution and the velocity probability distribution. This result is based on a new coupling of the process which gives a quantitative minorization condition and yields more insights on the convergence. In addition, we study on a toy model the dependency of the convergence rates on the dimension of the state space. Finally, we apply our results to the analysis of simulated annealing algorithms based on BPS.

==> quantitative_MC.tex <==
  \section{Quantitative contraction rates for Markov chains}
\label{app:quantitative_bounds}
In this section, we give for completeness a quantitative version of  \cite[Theorem 1.2]{HairerMattingly2011} which is used in \Cref{sec:metast-regime-anne}. Let $Q$ be a Markov operator on a smooth finite dimension manifold $\msm$ (in our applications $Q=P_{t_0}$ for some $t_0>0$, with $\msm= \R^{d} \times \msy$) and $V:\msm \to \coint{1,\plusinfty}$ (which can be thought as the one given by \eqref{eq:def_lyap_gene}). 
%If  $\mu_1$ and $\mu_2$ admit a density (still denoted $\mu_1$ and $\mu_2$) with respect to a measure $\dd x$ on $\msm$, then, equivalently,
%\begin{eqnarray*}
%\rho_\zeta(\mu_1,\mu_2) & = & \int ( 1+\zeta V(x)) |\mu_1(x)-\mu_2(x)|\dd x.
%\end{eqnarray*}

For any measurable function $\varphi : \msm \to \rset$ and $\zeta \geqslant 0$, we set
\begin{equation*}
\|\varphi\|_{\zeta,V}  =\underset{x\in \msm} \sup  \defEns  { \frac{|\varphi(x)|}{1+\zeta V(x)}} \eqsp,
\end{equation*}
and consider the weighted $V$-norm on $\mathcal P_{V}(\msm)=\{\mu\in\mathcal P(\msm) \, :\,  \mu(V) < \infty\}$, defined for $\mu_1, \mu_2 \in \mcp_{V}(\msm)$ by
\begin{equation}
  \label{eq:def_rho_zeta_D}
\rho_\zeta(\mu_1,\mu_2)  =  \sup\left\{ \mu_1( \varphi) - \mu_2( \varphi) \, : \,  \|\varphi\|_{\zeta,V} \leqslant 1\right\}.
\end{equation}

\begin{theorem}\label{thm:ThmCVexpo}
Suppose that there exist $\alpha,\gamma\in(0,1)$, $C_1>0$ and $C_2 > 2C_1$ such that for all $x,y,z \in \msm$, $V(x)+ V(y) \leq C_2$, 
\begin{equation*}
 \tvnorm{ Q(x,\cdot) -  Q(y,\cdot)} \leqslant 2( 1 - \alpha) \eqsp, \qquad QV(z) \leqslant  \gamma V(z) + C_1(1-\gamma)\eqsp.
\end{equation*} 
Then there exists $\zeta>0$ and $\kappa\in \ooint{0,1}$ such that for all $\mu_1,\mu_2\in\mathcal P_V( \msm)$,
\begin{equation*}
\rho_\zeta(\mu_1 Q,\mu_2 Q) \leqslant  \kappa \rho_\zeta(\mu_1,\mu_2) \eqsp,
\end{equation*}
where $\rho_{\zeta}$ is defined by \eqref{eq:def_rho_zeta_D}.
More precisely, if $C_2 = 4C_1$, then this holds with
%Consider some $\alpha_0\in(0,\alpha)$ and set
\begin{align*}
\zeta  = \alpha((1-\gamma)C_1)^{-1} \eqsp, \qquad \qquad \kappa  =  ( 1 - \alpha/ 2) \vee ( (3+\gamma)/4) \eqsp.
\end{align*}
\end{theorem}

\begin{proof}
 \cite[Lemma 2.1]{HairerMattingly2011} shows that 
\begin{equation*}
\rho_\zeta(\mu_1,\mu_2)  =  \sup\left\{ \mu_1( \varphi) - \mu_2 (\varphi) \, :\,   |\varphi |_{\zeta} \leqslant 1\right\} \eqsp,
\end{equation*}
where $\rho_\zeta$ is defined by \eqref{eq:def_rho_zeta} and
\begin{equation*}
 |\varphi |_{\zeta}  =  \underset{x\neq y}\sup\  \defEns{\frac{|\varphi(x) - \varphi(y)|}{2+ \zeta V(x) + \zeta V(y)} } =  \underset{c\in\R }\inf \| \varphi +c\|_{\zeta,V}.
\end{equation*}
Let $\varphi$ be a measurable function  such that $|\varphi |_{\zeta} = \| \varphi  \|_{\zeta,V} = 1$. We aim to show that $|Q \varphi |_{\zeta}\leqslant \kappa$ or, in other words, that
\begin{equation*}
|Q\varphi(x) - Q\varphi(y)|  \leqslant  \kappa ( 2 + \zeta V(x) + \zeta V(y)) 
\end{equation*}
for all $x,y\in \msm$.

First, consider the case where $V(x)+V(y) \geqslant C_2$. For $\zeta>0$, set
%Consider $\alpha_0 \in (0,\alpha)$, and set $\zeta = \frac{2(\alpha-\alpha_0)}{K}$ and  
 $\kappa_1 = \gamma + (1-\gamma)\frac{1+\zeta C_1}{1+ \zeta C_2/2}$. Note that $\gamma < \kappa_1 <1$, and 
%\[ \gamma + \frac{2K}{R} \ < \ \frac{2+\zeta R( \gamma + \frac{2K}{R})}{2+\zeta R} \ = \ \kappa_1 \ = \ 1 + \zeta \frac{R(\gamma-1)+ 2 K}{2+\zeta R}\ < \ 1.\]
%and that 
\[ 2(1-\kappa_1) + (\gamma - \kappa_1)\zeta C_2 + 2\zeta C_1(1-\gamma) \leqslant 0 \eqsp.\]
Hence,
\begin{align*}
&|Q\varphi(x) - Q\varphi(y)|  \leqslant   2 + \zeta QV(x) + \zeta QV(y)  \leqslant  2 + \zeta \gamma V(x) + \zeta \gamma V(y) + 2\zeta C_1  \\
& \leqslant  \kappa_1 ( 2 + \zeta  V(x) + \zeta  V(y)) + 2(1-\kappa_1) + (\gamma - \kappa_1)\zeta ( V(x) + V(y)) + 2\zeta C_1\\
& \leqslant  \kappa_1 ( 2 + \zeta  V(x) + \zeta  V(y)) \eqsp.
\end{align*}

Second, consider the case where $V(x)+V(y) \leqslant C_2$. Let $( Z_x, Z_y)$ be an optimal coupling of $Q(x,\cdot)$ and $Q(y,\cdot)$. % , in the sense that $Q\varphi(z) = \mathbb E[ \varphi(Z_z)]$, $z= x$ or $y$, and that
% \begin{equation*}
% \mathbb P( Z_x \neq Z_y )  =  (1/2)\frac12 \tvnorm{Q(x,\cdot) - Q(y,\cdot)}.
% \end{equation*}
Then, writing $\kappa_2 = ( 1 - \alpha +  \zeta C_1(1-\gamma)/2)  \vee \gamma$ (which is smaller than 1 for $\zeta$ small enough),
\begin{align*}
  |Q\varphi(x) - Q\varphi(y)| & \leqslant    \mathbb P( Z_x \neq Z_y ) \expe{ |\varphi(Z_x) - \varphi(Z_y)| |\ Z_x \neq Z_y}\\
& \leqslant  \mathbb P( Z_x \neq Z_y ) ( 2 + \zeta \, \expe{ V(Z_x) + V(Z_y) }) \\
& \leqslant  2 (1-\alpha) + \zeta\gamma ( V(x) + V(y)) + \zeta C_1 (1-\gamma)\\
& \leqslant   \kappa_2 ( 2 + \zeta V(x) + \zeta V(y) ) \eqsp,
\end{align*}
which concludes the general proof.

For $C_2=4C_1$, we chose $\zeta = \frac{\alpha}{(1-\gamma)C_1}$, so that $\kappa_2 = 1 - \alpha/2$ and
\[\kappa_1 \ = \ \gamma + (1-\gamma)\parenthese{ 1 - \frac{\alpha}{1-\gamma + 2\alpha}} \ = \ 1 - \frac{\alpha (1-\gamma)}{1-\gamma + 2\alpha} \eqsp. \]
Using that, for $a,b>0$,
\[ \frac{ab}{a+b} \ = \ \frac{a\wedge b}{1 + \frac{a\wedge b}{a\vee b}} \ > \ \frac{a\wedge b}2 \eqsp,\]
we get
\[\kappa_1 \ \leqslant \  1 - \frac{(2\alpha)\wedge (1-\gamma)}{4} =  ( 1 - \alpha/ 2) \vee ( (3+\gamma)/4)  \eqsp . \]
\end{proof}

Remark that, under the same assumptions that \Cref{thm:ThmCVexpo} but with $\alpha=0$, the same proof yields, for all $\zeta>0$ and all $\mu_1,\mu_2\in\mathcal P_V( \msm)$,
\begin{equation}
\label{eq:rmq-rho-beta}
\rho_\zeta(\mu_1 Q,\mu_2 Q)  \leqslant  (1+\zeta C_1) \rho_\zeta(\mu_1,\mu_2) \eqsp.
\end{equation}

% \begin{proof}[Proof of \Cref{theo:geo_ergo_gene}]
% From Corollary \ref{Corollary-lyap} and \Cref{lem:condition-doeblin}, \Cref{thm:ThmCVexpo} holds for $P_{t_0}$ for some $t_0>0$, with the function $V$ given by \eqref{eq:def_lyap_gene}. Let $\kappa$ and $\zeta$ be given by   \Cref{thm:ThmCVexpo} for $P_{t_0}$. Using \eqref{eq:rmq-rho-beta} we get, for $\nu_1,\nu_2\in\mathcal P_V(\R^{d}\times \msy)$ and $t\geqslant 0$,
% \begin{equation*}
% \Vnorm[\lyap]{\nu_1 P_t - \nu_2 P_t}   \leqslant  \frac1\zeta \rho_\zeta( \nu_1 ( P_{t_0})^{\lfloor t/t_0\rfloor}P_{t-t_0\lfloor t/t_0\rfloor},\nu_2( P_{t_0})^{\lfloor t/t_0\rfloor}P_{t-t_0\lfloor t/t_0\rfloor})\\
%  \leqslant  \frac{1+\zeta C_2}{\zeta }\kappa^{\lfloor t/t_0\rfloor}\rho_\zeta(\nu_1,\nu_2)\\
%  \leqslant  \frac{(1+\zeta C_2)(1+\zeta)}{\zeta\kappa }e^{t\ln \kappa/t_0 }\Vnorm[\lyap]{\nu_1   - \nu_2  }\eqsp.
% % \leqslant  e^{(t-1)\ln \kappa }(2 + \nu_1 V + \nu_2 V)\\
% % \leqslant  2 e^{(t-1)\ln \kappa }(2 + \nu_1 V ) \nu_2 V.
% \end{equation*}
% %In the particular case where $\nu_2 = \delta_{z}$ for $z=(x,y)\in\R^{2d}$, we bound
% %\begin{eqnarray}\label{\msmqBorneV}
% %  V(z) \ \leqslant \ e^{f(x)} + e^{\frac{|y|^2}{4\sigma^2}} \ \leqslant \  2 e^{f(x)+\frac{|y|^2}{4\sigma^2}} \ \leqslant \ 2 e^{c_4|x|+\frac{|y|^2}{4\sigma^2}} %( 1 + \frac{c_1+1}{\sqrt\delta}) e^{\frac14 U(x)} + e^{\frac{|y|^2}{4\sigma^2}} \ \leqslant \ 2( 1 + \frac{c_1+1}{\sqrt\delta}) e^{\frac14 U(x)+\frac{|y|^2}{4\sigma^2}}. 
% %\end{eqnarray}
% When $\nu_2 = \tpi$, by \cite[\Cref{prop:invarince-BPS}]{DurmusGuillinMonmarche:toolbox} , $\tpi P_t = \tpi$, and Conditions \eqref{ass:geo_erg_general_eq_1} and \eqref{ass:geo_erg_general_eq_4} ensures that $\tpi (\lyap) < \infty$. We bound
% \[ \Vnorm[\lyap]{\nu_1   - \tpi  } \ \leqslant \ \nu_1(V) + \tpi(V)\ \leqslant \ \nu_1(V)( 1 + \tpi(V)).\]
% Finally, note that the functions defined in \eqref{eq:def_lyap_gene} and \eqref{eq:lyap_thm_gene} are equivalent (their ratio is bounded above and below by positive constants), so that the associated $V$-norms are equivalent, which concludes.
% \end{proof}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_supplement"
%%% End:


==> simulated_proof.tex <==
\subsection{Proof of \Cref{thm:ThmRecuit}}
\label{sec:proof-simulated}
The semi-group $(P_{s,t})_{t \geq s \geq 0 }$ is associated with the family of generator $(\generator_{\beta(t)})_{t \geq 0}$ where for any $\beta >0$, $\generator_{\beta}$ is defined  for any  $f\in\mrc^1(\rset^d\times\msy)$ by
\begin{align}
\nonumber
&  \generator_{\beta} f(x,y) = \ps{y}{\nabla f(x,y)} + \beta (\ps{y}{\nabla U(x)})_+ \defEns{f(x,\Refl(x,y)) - f(x,y)} \\
    \label{eq:generator-recuit}
& \qquad   + \rate \defEns{\int_{\msy} f(x,w) \rmd \loiy(w)  - f(x,y)} \eqsp.
\end{align}
% Then, $\generator_{\beta} $ is the generator of a BPS process with refreshment law $\loiy$, refreshment rate $\rate$ and potential $U_\beta = \beta U$.  Consider $(\beta_t)_{t\geqslant0}$ a cooling schedule, which is to say a function $t\rightarrow \beta_t \geqslant 1$ which is increasing and goes to infinity at infinity. Then we can consider the inhomogeneous Markov process $(Z_t)_{t\geqslant 0}$ on $\rset^d\times\msy$ with generator $(\generator_{\beta_t})_{t\geqslant 0}$ and semi-group $( P_{s,t})_{0\leqslant s \leqslant t}$, such that for all $f\in L^\infty(\R^{2d})$ and all $0\leqslant s \leqslant t$,
% \begin{equation*}
%  P_{s,t} f(z) & =& \mathbb E( f(Z_t)\ |\ Z_s = z)
% \end{equation*}
% and for all $f\in \mathsf C^1(\rset^d\times\msy)$ and all $t\geqslant 0$,
% \[(\partial_s)_{|s=0}\co P_{t,t+s} f(z) \cf = \generator_{\beta_t}  f(z).\]%\hspace{15pt}\text{and} \hspace{15pt} \partial_s P_{s,t}^{(\beta)} f(z) = -L^{\beta_s} P_{s,t}^{(\beta)} f(z).\]
% The construction of the process is exactly the same as the homogeneous one presented in \Cref{sec:main-results}, except that \eqref{eq:def-temps-bounce} is now replaced by:
% \begin{equation*}
% T_{n+1}^{(2,\beta)} &=& \inf\ensemble{t \geq 0}{\int_0^t \beta_{\S^{(\beta)}_n+ s} \ps{Y^{(\beta)}_{\S^{(\beta)}_n}}{\nabla U (X^{(\beta)}_{\S^{(\beta)}_n}+s Y^{(\beta)}_{\S^{(\beta)}_n})}_+  \rmd s \geq E^{2}_{n+1}}.
% \end{equation*}
First, we establish a Foster-Lyapunov drift condition for $\generator_{\beta}$ uniformly on $\beta\geqslant1$.
\begin{lemma}
\label{lem:lyap-recuit}
Assume \Cref{ass:recuit}. There exist $A_1,A_2,A_3>0$, $\beta_*\geqslant 1$ and $V_1,V_2\in \mrc^1(\rset^d\times\msy)$, with $V_i \exp(-U/2)$ bounded above and below by positive constants for $i=1,2$, such that for all $\beta\geqslant \beta_*$,
\begin{equation*}
\generator_{\beta} V_1  \leqslant  A_1( A_2 - V_1) \eqsp,
\end{equation*}
and for all $\beta \geqslant 1$,
\begin{equation*}
\generator_{\beta} V_2  \leqslant  A_3  V_2  \eqsp.
\end{equation*}
\end{lemma}
\begin{proof}
  We check that \Cref{ass:geo_erg_general}  holds for $\beta$ large enough, with $\bU = U/2$ and the potential  $x \mapsto  U_{\beta}(x)$. Indeed, set  $\ell(x) = 1$ for all $x\in\rset^d$ and $H(t) = t^2$ for $t\in\rset$. Then all the conditions of \Cref{ass:geo_erg_general}  are clearly satisfied, with $c_1$, $c_2$ and $c_4$ which does not depend on $\beta$, and $c_3 = \beta$. Let $\beta_*$ be large enough so that \eqref{eq:condition_geo_4} holds for $\beta \geqslant \beta_*$ and $\kappa$ defined in \eqref{eq:def_kappa} is equal to $1$.

Let $\lyap_1$ be the function defined by \eqref{eq:def_lyap_gene}. According to \Cref     {lem:lyapunov}, there exist $A_1,A_2>0$ such that
     \begin{equation*}
\generator_{\beta_*} V_1  \leqslant  A_1( A_2 - V_1).
\end{equation*}
Now, for $\beta \geqslant \beta_*$, keeping the notations of \Cref{sec:Lyapunov},
\[( \generator_{\beta} - \generator_{\beta_*}) V_1(x,y)  \ = \ (\beta-\beta_*)e^{ U(x)/2}\ps{y}{\na U(x)}_+( \varphi(-\theta) - \varphi(\theta) ) \ \leqslant \ 0\eqsp.\]

Second, set for any $(x,y)\in \rset^d\times \msy$, $V_2(x,y) = \exp(U(x) /2)   \varphi_2( \ps{y}{ \na U(x)}  )$, where $\varphi_2\in\mrc^1(\rset)$ is an increasing function such that $\varphi(s) = 1$ for $s\leqslant -1$ and $\varphi(s)=3$ for $s\geqslant 1$. Then, for all $\beta\geqslant 1$, 
\begin{align*}
e^{-  U(x)/2}\generator_{\beta} V_2(x,y) & \leqslant    \ps{y}{ \na U(x)} \varphi_2( \ps{y}{ \na U(x)}  ) + M^2 \norm{\na^2 U}_\infty  \norm{\varphi_2'}_\infty + 2\rate \\
&  + \beta \ps{y}{\na U(x)}_+\defEns{ \varphi( - \ps{y}{ \na U(x)}) - \varphi( \ps{y}{ \na U(x)} ) } \\
& \leqslant  3 + M^2 \norm{\na^2 U}_\infty  \norm{\varphi_2'}_\infty + 2\rate\eqsp,
%\frac12 \ps{y}{ \na U(x)} + M^2 \norm{\na^2 U}_\infty + \rate + \ps{y}{\na U(x)}_+  \varphi\co - \ps{y}{ \na U(x)} \cf
\end{align*}
and we conclude by noting that $\exp(U(x)/2)\leqslant V_2(x,y)$ for any $(x,y) \in \rset^d \times \msy$.
%When $\ps{y}{ \na U(x)} \geqslant 2$, $\varphi\co - \ps{y}{ \na U(x)} \cf =  -1$, so that for all $(x,y)\in \rset^d\times \msy$,
%\[\generator_{\beta} V_2(x,y)\ \leqslant\  ( 1 + M^2 \norm{\na^2 U}_\infty + \rate ) e^{ U(x)} \ \leqslant\  ( 1 + M^2 \norm{\na^2 U}_\infty + \rate )  V_2(x,y)\eqsp.\]
\end{proof}

\begin{corollary}
\label{corollary-recuit}
Assume that the assumptions of \Cref{thm:ThmRecuit} hold. Then there exists $A_4>0$ such that for all $t,s\geqslant 0$ and $(x,y) \in \rset\times \msy$,
\begin{equation*}
P_{t,t+s} V_1(x,y)  \leqslant  A_4 e^{A_3 s}V_1(x,y)\eqsp,
\end{equation*}
and for all $t\geqslant 0$ such that $\beta(t)\geqslant \beta_*$,
\begin{equation*}
P_{t,t+s} V_1(x,y)  \leqslant  e^{-A_1 s} V_1(x,y) + ( 1 - e^{-A_1 s} ) A_2\eqsp,
\end{equation*}
where $V_1 \in \rmc^1(\rset^d \times \msy)$, $A_1,A_2,A_3$ are given by \Cref{lem:lyap-recuit}. 
\end{corollary}
\begin{proof}
The proof follows the same line as  the proof of \Cref{Corollary-lyap}, using \Cref{lem:lyap-recuit} and $V_1/V_2$ is bounded above and below by positive constants.
\end{proof}

%
%
%In this section, we consider $U\in\mathsf C^2(\R^d)$ which satisfies Assumption \ref{HypThm} and, for an inverse temperature $\beta>0$, we denote by $P_t^{(\beta)}$ the semi-group associated to a BPS in $\R^{2d}$ with refreshment rate $r>0$, variance $\sigma^2>0$ and potential $U_\beta = \beta U$. We are interested in the small temperature regime, namely $\beta\rightarrow\infty$.

%Denoting by $L^{(\beta)}$ the generator of $P_t^{(\beta)}$  and considering $V$ the function defined in Section \ref{SectionLyapunov} (associated to $U$, and not to $\beta U$), we remark that, for $\beta\geqslant 1$,
%\begin{eqnarray}\label{EqLyapunovRecuit}
%  L^\beta V(x,y) - L V(x,y)\notag \\
% = (\beta - 1) ( y\cdot \na U(x))_+ ( \varphi ( -y\cdot\na U(x))- \varphi ( y\cdot\na U(x))) e^{\frac14 U(x)} R(x,y)\chi( U(x)) \notag\\
% \leqslant  0. 
%\end{eqnarray}
%Hence,
%\begin{equation*}
%P_t^\beta V(z)  \leqslant  V(z) e^{-\frac r2 t} +  C( 1- e^{-\frac r2 t})
%\end{equation*}
%with $C$ given in Lemma \ref{LemLyapunov} which, in particular, does not depend on $\beta$. The compact $\mathsf K_2 = \{ V \leqslant 4C\}$ is included in $\mathsf D_R\times \mathsf D_R$ with $R>0$ that does not depend on $\beta$. Following the proof of Lemma \ref{LemCouplageCompact} and its notations, we see that there exists $\bar \chi>0$ that does not depend on $\beta$ such that
%\begin{equation*}
%\mathbb P( T_c < 1)  \geqslant  \bar \chi e^{-\beta A_R} 
%\end{equation*}
%where $A_R$ is given by \eqref{EqDefCr} (and does not depend on $\beta$). Hence, following the proof of Theorem~\ref{ThmMain}, we can check that the following has been established:
%\begin{prop}\label{PropMetastable}
%For all $\sigma,r>0$ and $U\in\mathsf C^2(\R^d)$ which Assumption \ref{HypThm}, there exists $\lambda,t_0,\theta>0$ such that for all $\beta\geqslant 1$, $t\geqslant t_0$ and $z\in  \R^{2d} $,
%\begin{equation*}
%\| \delta_z P_t^\beta - \mu_\beta\|_1  \leqslant   2 e^{-\lambda e^{-\beta \theta} (t-t_0) + \frac{U(x)}{4} + \frac{|y|^2}{4\sigma^2}},
%\end{equation*}
%where $\mu_\beta(\dd x,\dd y) = \rmZ_\beta^{-1} e^{-\beta U(x) + \frac{1}{2\sigma^2}|y|^2}\dd x\dd y$ and $\rmZ_\beta$ is the normalization constant.
%\end{prop}
%The rate of convergence $\lambda e^{-\beta \theta}$ that we obtain goes exponentially fast to 0 as $\beta$ goes to infinity: in fact, when $U$ admits several local minima, this is the expected order of magnitude. More precisely, the optimal $\theta$ such that this holds should be the critical depth of the potential (see \cite{MonmarcheRTP}), but in order to prove this, in Lemma \ref{LemCouplageCompact}, we should try to couple the processes after several jump (instead of just one) by making them follow  broken line trajectories close to an optimal path (a path with minimal height) between the initial positions. Since the critical depth of a potential is unknown in practice, this would not change much from the result of Proposition \ref{PropMetastable}. At small temperature (large $\beta$), the process stays for very long times in the vicinity of local minima of $U$: the process is said metastable. For more considerations on metastability for the BPS, see \cite{MonmarcheRTP}.
%
%\bigskip
%%
%%We are also able to prove a result similar to \cite[Theorem 1.5]{MonmarcheRTP} in the case of an annealing procedure. Consider $(\beta_t)_{t\geqslant0}$ a cooling schedule, which is to say a function $t\rightarrow \beta_t>1$ which is increasing and goes to infinity at infinity. Then we can consider the inhomogeneous Markov process $Z^{(\beta)}$ with generator $(L^{\beta_t})_{t\geqslant 0}$ and semi-group $( P_{s,t}^{(\beta)})_{0\leqslant s \leqslant t}$, such that for all $f\in L^\infty(\R^{2d})$ and all $0\leqslant s \leqslant t$,
%%\begin{equation*}
%% P_{s,t}^{(\beta)} f(z)  = \mathbb E( f(Z_t)\ |\ Z_s = z)
%%\end{equation*}
%%and for all $f\in \mathsf C^\infty$ with compact support,
%%\[\partial_t P_{s,t}^{(\beta)} f(z) = L^{\beta_t} P_{s,t}^{(\beta)} f(z).\]%\hspace{15pt}\text{and} \hspace{15pt} \partial_s P_{s,t}^{(\beta)} f(z) = -L^{\beta_s} P_{s,t}^{(\beta)} f(z).\]
%%The construction of the process is exactly the same as the homogeneous one, except that \eqref{EqDefTempsBounce} is now replaced by:
%%\begin{equation*}
%%T_1  = \inf\left\{ t>t_k, \ E_k < \int_{0}^{t-t_k} \beta_{t_k+s}( Y^{(\beta)}_{t_k} \cdot \na U( X^{(\beta)}_{t_k} + s Y^{(\beta)}_{t_k} ))_+ \dd s\right\}.
%%\end{equation*}
%%
%%\bigskip
%
%For the sake of simplicity, suppose that the cooling schedule is piecewise constant, and more precisely that there exists $t_1 >0$ such that $\beta_t =  \beta_{nt_1}$ for all $t\in [nt_1,(n+1)t_{1})$. In the following, we denote $t_n = nt_1$, $\beta_n = \beta_{t_n}$, $Q_n = P_{t_1}^{\beta_n}$, $\mu_n=\mu_{\beta_n}$, so that, if $n=\lfloor t/t_1\rfloor$ then
%\begin{equation*}
%P_{0,t}^{(\beta)}  = Q_0 Q_1 \cdots Q_{n-1} P_{t-t_n}^{\beta_{n}} .
%\end{equation*}
%
%
%\bigskip
%
%Note that, as $\beta$ goes to infinity, the mass of $\mu_\beta$ concentrates on the vicinity of the global minima of $U$. The aim of the simulated annealing algorithm is to ensure that the process $Z_t^{(\beta)}$ get and stays close to its instantaneous equilibrium, namely the equilibrium of $L^{\beta_t}$, which is $\mu_{\beta_t}$, so that $Z_t^{(\beta)}$ itself converges to the global minima of $U$. It is well known that this can be achieved if $\beta_t$ goes to infinity sufficiently slowly. Indeed, we will prove this below (Theorem~\ref{ThmRecuit}).


\begin{lemma}
\label{lem:couplage-recuit}
Assume that the assumptions of \Cref{thm:ThmRecuit} hold. Then, for all compact set $\mathsf K$ of $\R^{d}\times \msy$, there exist $s_1,\chi,A_5>0$  which depend on $\mathsf K$, $\loiy$, $\rate$ and $U$ but not on $t \mapsto \beta(t)$, such that for all  $(x,y),(\tx,\ty)\in\mathsf K$, all $t\geqslant 0$ and all $s\geqslant s_1$, %denoting by $\delta_{z}$ the Dirac mass at $z$, 
\begin{equation*}%\label{EqCouplageCompact}
 \tvnorm{ P_{t,t+s}((x,y),\cdot) -  P_{t,t+s} ((\tx,\ty),\cdot)} \leq 2\parentheseDeux{1 - \chi \exp \parenthese{ - A_5 \int_{t}^{t+s} \beta(u) \rmd u }} \eqsp. 
\end{equation*}
\end{lemma}
\begin{proof}
The arguments are exactly those of the proof of \Cref{lem:condition-doeblin-precis}, hence of \cite[Theorem 5.1]{MonmarcheRTP}, so that we only give a sketch of proof. First, considering the case $\beta=0$, we have already shown in \Cref{sec:couplage} that, starting from two different points in a given compact $\mathsf K$, it is possible to merge two processes in a time $s_1>0$ while staying in a compact $\mathsf K'$, with some probability $\chi>0$. Call $\mathsf E$ this event. Then, considering the case $\beta>0$, we follow the same coupling up to the first bounce time. The processes have merged if this first bounce happens after time $s_1$, which occurs with probability 
\begin{multline*}
\probaCond{ \int_t^{t+s_1} \beta(u) \ps{Y^{(\beta)}_{u}}{\nabla U (X^{(\beta)}_{u})}_+  \rmd u \geqslant E^{2}_{1} } {\mse}  \\ \geq  \exp \parenthese{ - M\norm{\nabla U}_{\infty, K'}\int_{t}^{t+s_1} \beta(u) \rmd u }\eqsp,
\end{multline*}
where $M = \sup_{(w,z) \in \msk'} \norm{z}$.
\end{proof}

Let $V_1$ and $A_i$, $i\in \{1,\ldots,4\}$, be given by Corollary \ref{corollary-recuit}. Then, let $s_1,\chi,A_5>0$ be given by \Cref{lem:couplage-recuit}, with $\mathsf K = \{(x,y)\in\rset^d\times\msy,\ V_1(x) \leqslant 2 A_2\}$. Let
\begin{equation}
  \label{eq:def_t_0}
  t_0 = \inf\{t\geqslant 0,\ \beta(t) \geqslant \beta_* \} \eqsp,
\end{equation}
and for $t\geqslant t_0$, define
\begin{equation}
  \label{eq:def_bfn}
 \bfn(t)= \lfloor (t-t_0)/s_1\rfloor\eqsp.
\end{equation}
Consider the following decomposition,
\begin{equation*}
P_{0,t}   = P_{0,t-\bfn(t) s_1}Q_0Q_1   \cdots  Q_{\bfn(t)-1} Q_{\bfn(t)} \eqsp, 
\end{equation*}
where $Q_0$ is the identity kernel and for $k\in \{ 1 ,\ldots, n(t)\}$, we set
\begin{equation}
  \label{eq:def_q_k}
  Q_k = P_{t- (\bfn(t)-k+1)s_1,t-(\bfn(t)-k)s_1} \eqsp.
\end{equation}
For any measurable function $\varphi : \rset^d \times \msy \to \rset$ and $\zeta \geqslant 0$, we set
\begin{equation*}
\|\varphi\|_{\zeta,V_1}  =\underset{(x,y)\in \rset^d \times \msy} \sup  \defEns  { \frac{|\varphi(x,y)|}{1+\zeta V_1(x)}} \eqsp,
\end{equation*}
and consider the weighted $V_1$-norm on $\mathcal P_{V_1}(\rset^d \times \msy)=\{\mu\in\mathcal P(\rset^d \times \msy) \, :\,  \mu(V_1) < \infty\}$, defined for $\mu_1, \mu_2 \in \mcp_{V_1}(\rset^d \times \msy)$ by
\begin{equation}
  \label{eq:def_rho_zeta}
\rho_\zeta(\mu_1,\mu_2)  =  \sup\left\{ \mu_1( \varphi) - \mu_2( \varphi) \, : \,  \|\varphi\|_{\zeta,V_1} \leqslant 1\right\}.
\end{equation}
Note that $\rho_\zeta(\mu_1,\mu_2) $ increases with $\zeta$ and that $\rho_0 = \tvnorm{\cdot}$. In addition, for any $\mu_1,\mu_2 \in  \mcp_{V_1}(\rset^d \times \msy)$,
\begin{equation*}
  \rho_\zeta(\mu_1,\mu_2) \leq \Vnorm[V_1]{\mu_1-\mu_2} \leq (1+\zeta)^{-1} \rho_\zeta(\mu_1,\mu_2) \eqsp.
\end{equation*}
\begin{lemma}
  \label{lem:convergence}
  Assume that the conditions of \Cref{thm:ThmRecuit} hold. Then for all $\nu_1,\nu_2\in\mcp_{V_1}(\R^{d} \times \msy)$, $t \geq t_0$ and  all $k\in \{1,\ldots,\bfn(t)\} $,
\begin{equation}\label{eq:recuit-contraction}
\rho_{\epsilon_k}( \nu_1 Q_k,\nu_2 Q_k )  \leqslant  \kappa_k  \rho_{\epsilon_k}( \nu_1 ,\nu_2 ) \eqsp,
\end{equation}
where 
\begin{align*}
   \epsilon_k  &=  \frac{  \chi  }{(1-\gamma)A_2}   \exp \parenthese{ - A_5 \int_{t-(n-k+1)s_1}^{t-(n-k)s_1} \beta_u \rmd u } \eqsp,\\
\kappa_k & =  1 - \parenthese{ \frac{\chi}2 \wedge \frac{1-\gamma}{4}} \exp \parenthese{ - A_5 \int_{t-(n-k+1)s_1}^{t-(n-k)s_1} \beta_u \rmd u }\eqsp,  \gamma &= \exp(-s_1 A_1) \eqsp.
\end{align*}
\end{lemma}
\begin{proof}
  It is a direct application  to $Q_k$ for all $k$ of   \Cref{thm:ThmCVexpo} based on \Cref{lem:couplage-recuit} and  \Cref{corollary-recuit}.
\end{proof}
 
For a fixed $\beta\geqslant 0$,  let $(P_t^{(\beta)})_{t\geq 0}$ be the semi-group of the BPS sampler associated with  the potential $x \mapsto \beta U(x)$ and, for $t\geqslant t_0$ and  $k\in\{0,\ldots,\bfn(t)\}$, let
\begin{equation}
  \label{eq:def_Q_'}
  Q'_k = P_{s_1}^{(\beta_{k})} \eqsp,
\end{equation}
where for ease of notation simplicity we denote
\begin{equation}
  \label{eq:def_beta_k}
  \beta_k = \beta_{t-(\bfn(t)-k)s_1} \eqsp.
\end{equation}
 In other words, $Q'_k$ is similar to $Q_k$ except that the inverse temperature is frozen. Let $\tpi_k$ be the invariant measure of $Q'_k$, namely 
\[\tpi_k  =   \pi_k\otimes \loiy\eqsp,\]
where $\pi_k$ admits a density with respect to the Lebesgue measure given for any $x \in \rset^d$ by
\[\pi_k( x) =  \rmZ_k^{-1} \exp (-\beta_{k} U(x)) \rmd x  \eqsp, \qquad \rmZ_k = \int_{\rset^d}\exp (-\beta_{k} U(\tx)) \rmd \tx\eqsp.\]


We know that the mass of $\pi_k$ concentrates, as $k\rightarrow \infty$, around the vicinity of the global minima of $U$. To get the same with $ P_{0,t}((x,y),\cdot)$, we need to show that $\tvnorm{\tpi_{\bfn(t) }- P_{0,t}((x,y),\cdot)}$ vanishes as $t\rightarrow\infty$. Denoting, for $t\geqslant t_0$ and $k\in\{0,\ldots,\bfn(t)\}$, $\nu_{k} = \updelta_{(x,y)} P_{0,t-\bfn(t)s_1}Q_0Q_1   \cdots  Q_{k-1} Q_{k}$, where $Q_k$ is defined in \eqref{eq:def_q_k}, it is then natural to study
\begin{equation}
  \label{eq:def_an}
  u_k = \rho_{\epsilon_k}( \nu_k,\tpi_k)\eqsp.
\end{equation}
From \eqref{eq:recuit-contraction}, for any $t \geq t_0$, $k \in \{1,\ldots,\bfn(t)\}$
\begin{eqnarray}\label{eq:recuit-an-en}
u_k  \leqslant  \kappa_k  \rho_{\epsilon_k}( \nu_{k-1},\tpi_{k-1} ) + \rho_{\epsilon_k}( \tpi_{k-1} Q_k,\tpi_{k} ) \ \leqslant \ \kappa_k u_{k-1} + e_k 
\end{eqnarray}
where 
\begin{equation*}
e_k = \rho_{\epsilon_k}( \tpi_{k-1} Q_k,\tpi_{k} )
\end{equation*}
and used that $\rho_{\epsilon_k}( \nu_{k-1},\tpi_{k-1} )  \leqslant \rho_{\epsilon_{k-1}}( \nu_{k-1},\tpi_{k-1} ) $ since  $(\epsilon_k)_{k \geq 0}$ is non-increasing.

%
%First, without assuming anything concerning the $\beta_n$'s, note that the remarks that led to Proposition \ref{PropMetastable} still applies here and, together with Theorem \ref{ThmCVexpo}, yield:
%
%\begin{lem}\label{LemRecuit1}
%Let $\gamma = \rme^{-\frac{rt_1}{2}}$, and $V,C$ be given in Lemma \ref{LemLyapunov}. Then, there exist $\bar \chi,\theta>0$ such that, denoting
%\begin{equation*}
%\epsilon_n  = \frac{\bar \chi \rme^{-\theta\beta_{n}}}{(1-\gamma)C} \wedge 1\\
%\kappa_n  =  1 - \frac{\bar \chi \rme^{-\theta\beta_{n}}}2,
%\end{equation*}
%and considering the distance $\rho_n=\rho_{\epsilon_n}$ on $\mathsf P_V(\R^{2d})$ such as defined in Section \ref{SectionDemoThmMain}, then we have, for all $\nu_1,\nu_2\in\mathsf P_V(\R^{2d})$ and for all $n\in\mathbb N$,
%\begin{equation*}
%\rho_{n}( \nu_1 Q_n,\nu_2 Q_n )  \leqslant  \kappa_n  \rho_{n}( \nu_1 Q_n,\nu_2 Q_n ).
%\end{equation*}
%\end{lem}
%
%We will also make use of the following:
\begin{lemma}\label{lem:recuit-en}
Assume that the conditions of \Cref{thm:ThmRecuit} hold. Then, there exists $A_6>0$ such that for all $t\geqslant t_0$, all $k \in \{ 1,\ldots, \bfn(t)\}$ and $l\geqslant 1$, there exists $A_l>0$ such that
\begin{equation*}
e_k  \leqslant  A_l (  \sqrt{\beta_{k} - \beta_{k-1}} + \beta_k - \beta_{k-1} )  + A_6  \rme^{-\frac12( \beta_{k-1}-1) l}\eqsp,
\end{equation*}
where $\beta_k$, $\bfn$ and $t_0$ are defined by \eqref{eq:def_beta_k}, \eqref{eq:def_bfn} and \eqref{eq:def_t_0} respectively.
\end{lemma}
\begin{proof}
Let $t \geq t_0$, $k\in \{1,\ldots,\bfn(t)\}$ and $l \geq 1$.
  In the proof, $C$ stands for a constant which may change from line to line but does not depend on $k$, $l$ and $\beta$.
We bound 
\begin{eqnarray}\label{eq:borne-en-recuit}
e_{k}  \leqslant  \rho_{\epsilon_k}( \tpi_{k-1} ,\tpi_{k} ) + \rho_{\epsilon_k}( \tpi_{k-1} Q_{k},\tpi_{k-1} )
\end{eqnarray}
and deal with each terms of the right hand side  apart.
% Writing $\rmZ_{k} = \int \rme^{-\beta_{k} U(w)}\dd w$ and $\mu_{k}$ the Lebesgue density of $\mu_{k}$, from \eqref{EqBorneV},
Indeed, for the first one, the first marginal of $\tpi_{k-1}$ and $\tpi_{k}$ having an explicit density, and their second marginal being equal, we bound
\begin{align}
  \nonumber
 \rho_{\epsilon_k}( \tpi_{k-1} ,\tpi_{k} ) & =  \int_{\rset^d\times\msy} ( 1 + \epsilon_{k} V_1(x,y)) |\pi_{k}(x) - \pi_{k-1}(x)| \rmd x \loiy(\rmd y)\\
  \nonumber
                                           & \leqslant   C\int_{\rset^d} \rme^{U(x)/2} \left|\frac{\rme^{-\beta_{k} U(x)}}{\rmZ_{k}} - \frac{\rme^{-\beta_{k-1} U(x)}}{\rmZ_{k-1}} \right|\dd x\\
    \nonumber
                                           & \leqslant  C \rme^{ l/2}\int_{\rset^d} \left|\frac{\rme^{-\beta_{k} U(x)}}{\rmZ_{k}} - \frac{\rme^{-\beta_{k-1} U(x)}}{\rmZ_{k-1}} \right|\dd x\\
  \label{eq:recuit_1}
&   + C \int_{\{U>l\}} \frac{\rme^{-(\beta_{k}-\frac12) U(x)}}{\rmZ_{k}} + \frac{\rme^{-( \beta_{k-1}-\frac12) U(x)}}{\rmZ_{k-1}} \dd x\eqsp.
\end{align}
We treat the two terms in the right-hand-side apart. 
The first term is the  total variation distance between  $\pi_{k}$ and $\pi_{k-1}$. Since $\beta_{k-1} \leq \beta_k$ since $\beta$ is non-decreasing, $\rmZ_{k-1} \geqslant \rmZ_{k}$. Using  Pinsker's inequality and this result, we get
\begin{align}
  \nonumber
  \parenthese{ \int_{\rset^d} \left|\frac{\rme^{-\beta_{k} U(x)}}{\rmZ_{k}} - \frac{\rme^{-\beta_{k-1} U(x)}}{\rmZ_{k-1}} \right|\dd x }^2 &\leqslant   2
                                                                                                                                             \int_{\rset^d} \ln\parenthese{ \frac{\rme^{-\beta_{k-1} U(x)}\rmZ_{k}}{\rme^{-\beta_{k} U(x)}\rmZ_{k-1}}  } \pi_{k-1}(x) \rmd x \\
    \nonumber
                                                                                                                                           &\leqslant  2 ( \beta_{k} - \beta_{k-1}) \int_{\rset^d} U(x) \frac{\rme^{-\beta_{k-1} U(x)}}{\rmZ_{k-1}} \dd x\\
    \nonumber
& \leqslant   2  ( \beta_{k} - \beta_{k-1}) ( 1 + C \sqrt{\beta_{k-1}} \rme^{-\beta_{k-1}+1} ) \\
\label{eq:recuit_masse_0}
                                                                                                                                         & \leqslant   C  ( \beta_{k} - \beta_{k-1})\eqsp,
\end{align}
where we used for the two last inequalities that 
\[\int_{\{U>1\}} U(x) \rme^{-U(x)}  \dd x \ \leqslant \ 2 \int_{\rset^d}   \rme^{-U(x)/2}  \dd x\ < \ \infty\]
and since $U(0) = 0$, $U(x) \leq \norm{\nabla^2 U}_{\infty} \norm{x}^2$, for any $x \in \rset^d$ by \Cref{ass:recuit}, 
\[\rmZ_{k-1} \ \geqslant \ \int_{\rset^d} \rme^{- \beta_{k-1} \|\na^2 U\|_\infty \norm[2]{x}} \rmd x \ \geqslant\ C \beta_{k-1}^{-d/2} >0 \eqsp.\]
%where we used that $\min U = 0$ and Laplace's method (possibly at a higher level, if all the global minima of $U$ have degenerated Hessian). % (possibly bounding $U(x)\leqslant U(x) + m (x-x_0)^2=W(x)$ with $U(x_0)=0$, so that $W$ admits a unique global minimum).

Similarly, for the second term of \eqref{eq:recuit_1} we obtain %denoting by $vol$ the Lebesgue volume of a set,
\begin{equation*}
 \int_{\{U>l\}} \frac{\rme^{-(\beta_{k}-\frac12) U(x)}}{\rmZ_{k}}  \dd x \leqslant   C \beta_k^{d/2}\rme^{-(\beta_{k}-1)l} \int_{\rset^d} \rme^{- U(x)/2} \rmd x\eqsp.
 %\frac{\int_{U>l}\rme^{- ( \frac{\beta_{k}}{2}-\frac14) U(x)}\dd x }{vol(U<l/2)}\\
 %  \leqslant  \frac{\rme^{-   \frac{\beta_{k} l}{8} }\int \rme^{-  \frac{\rho}{16}|x|^2}\dd x }{vol(U<l_0/2)}.
\end{equation*}
Using that for any $t \geq 1$, $t^{d/2}\exp(-l(t-1)/2) \leq  (d/l)^{d/2}\exp(-(d-l)/2)$ if $d \geq \ell$ and $t^{d/2}\exp(-l(t-1)/2) \leq 1$ otherwise, there exists $A_{6,1}$ which does not depend on $l$ such that 
\begin{equation}
  \label{eq:recuit-masse}
 \int_{\{U>l\}} \frac{\rme^{-(\beta_{k}-\frac12) U(x)}}{\rmZ_{k}}  \dd x \leq A_{6,1} \rme^{-(\beta_{k}-1)l/2} \eqsp.
\end{equation}
Combining this bound and~\eqref{eq:recuit_masse_0} in \eqref{eq:recuit_1}, we get that there exists $A_{l,1} \geq 0$ such that  
\begin{equation}
  \label{eq:recuit_first_bound_main_lemma}
   \rho_{\epsilon_k}( \tpi_{k-1} ,\tpi_{k} ) \leq A_{l,1}\sqrt{\beta_k-\beta_{k-1}} + A_{6,1} \rme^{-(\beta_k-1)l/2} \eqsp.
\end{equation}

The second term of \eqref{eq:borne-en-recuit} is treated through a synchronous coupling similar to \cite[Proposition 11]{DurmusGuillinMonmarche:toolbox}. Indeed, $\tpi_{k-1}$ being invariant for $Q'_{k-1}$ defined in \eqref{eq:def_Q_'} and by \eqref{eq:def_rho_zeta},
\begin{align}
\nonumber
  \rho_{\epsilon_{k}}( \tpi_{k-1} Q_{k},\tpi_{k-1} )& = \rho_{\epsilon_{k}}( \tpi_{k-1} Q_{k},\tpi_{k-1}Q_{k-1}' )\\
  \label{eq:bound_rho_eps_k}
 & =  \underset{\norm{\varphi}_{\epsilon_{k},V_1}\leqslant 1}\sup\left\{ \mathbb E[ \varphi( X_{s_1},Y_{s_1}) - \varphi( X_{s_1}',Y_{s_1}')]\right\}\eqsp,
\end{align}
where $(X_t,Y_t)_{t\geqslant0}$ (resp. $(X_t',Y_t')_{t\geqslant0}$) is a BPS process with a fixed temperature $\beta_{k-1}$ (resp. a annealed BPS process with  cooling schedule $s \mapsto \beta(t-(\bfn(t)-k+1)s_1 +s)$) and $(X_0,Y_0) = (X_0',Y_0')$ is distributed according to  $\tpi_{k-1}$. Following \cite[Proposition 11]{DurmusGuillinMonmarche:toolbox}, we construct such processes in such a way $(X_t,Y_t) = (X_t',Y_t')$ up to time $T^{'}_{\rmb}$, where $T^{'}_{\rmb}$ is the first time $(X_t',Y_t')_{t \geq 0}$ bounces while $(X_t,Y_t)_{t \geq 0}$ does not, defined by
\begin{equation*}
T^{'}_{\rmb} =  \inf\left\{\tau \geqslant 0,\ E < \int_0^\tau ( \beta_{k} - \beta_{t-(\bfn(t)-n)s_1 + s}) \ps{Y^{(\beta)}_s}{\nabla U(X^{(\beta)}_s)}_+ \rmd s\right\}\eqsp,
\end{equation*}
where $E$ is a standard exponential random variable independent of $Z$.



Consider the compact sets $\mathsf K = \{(x,y)\in\rset^d\times\msy \, : \, U(x)<l\}$ and $\tmsk = \{(x,y) \in\rset^d\times\msy \, : \, \dist((x,y),\msk) \leq M s_1\}$, where $\dist(\cdot,\msk)$ is the distance from $\msk$ and $M = \sup_{z \in \msy} \norm{z}$. That way, if a BPS with refreshment law $\loiy$ over $\msy$ have an initial condition in $\mathsf K$, then on the time interval $[0,s_1]$ it necessarily stays in $\tmsk$.
 
Consider $\varphi:\rset^d\times \msy : \rightarrow\rset$ with $\norm{\varphi}_{\epsilon_{n+1},V_1}\leqslant 1$ and the following decomposition
\begin{align}
  \nonumber
  \mathbb E[ \varphi( X_{s_1},Y_{s_1}) - \varphi( X_{s_1}',&Y_{s_1}')] =  \mathbb E[\1_{\msk}(X_0,Y_0)\{ \varphi( X_{s_1},Y_{s_1}) - \varphi( X_{s_1}',Y_{s_1}')\}] \\ & +  \mathbb E[\1_{\rset^d \times \msy \setminus \msk}(X_0,Y_0)\{ \varphi( X_{s_1},Y_{s_1}) - \varphi( X_{s_1}',Y_{s_1}')\}] \eqsp.
\label{eq:decomp_recuit}
\end{align}
We bound the two terms separately. First, using that if $(X_0,Y_0) \in \msk$, then for any $t \in \ccint{0,s_1}$, $(X_t',Y_t') \in \tmsk$, we have 
 \begin{align}
\nonumber
      \mathbb E[ \1_{\msk}(X_0,Y_0) & \{\varphi( X_{s_1},Y_{s_1}) - \varphi( X_{s_1}',Y_{s_1}')\}]\\
\nonumber
   =   2 ( 1 + \epsilon_1)& \| V_1\|_{\infty, \tmsk} \proba{(X_0,Y_0) \in \msk, (X_{s_1},Y_{s_1}) \neq (X_{s_1}',Y_{s_1}')}\\
   \nonumber
   =   2 ( 1 + \epsilon_1) &\| V_1\|_{\infty, \tmsk} \proba{(X_0,Y_0) \in \msk, T'_{\rmb} < s_1} \\
\nonumber
    \leqslant   2 ( 1 + \epsilon_1) & \| V_1\|_{\infty, \tmsk}  \proba{ E < M \norm{\na U}_{\infty,\tmsk} \int_0^{s_1} ( \beta_{k} - \beta_{t-(\bfn(t)-n)s_1 +s})  \rmd s}\\
   \label{eq:first_bound_decomp_recuit}
 & \leqslant   2 ( 1 + \epsilon_1) \| V_1\|_{\infty, \tmsk}  M \norm{\na U}_{\infty,\tmsk} s_1 ( \beta_{k} - \beta_{k-1})   \eqsp,
 \end{align}
 where $M = \sup_{z \in \msy}\norm{z}$.
 % and
 % \begin{align*}
 % \mathbb P ( T^{'}_{\rmb} < s_1) & 
 % \end{align*}
Note that $\norm{\na U}_{\infty,\tmsk} $ depends on $\tmsk$, hence on $l$.
 
 Next using \Cref{lem:lyap-recuit} and the Markov property, we get
 \begin{align*}
  \mathbb E[\1_{\rset^d \times \msy \setminus \msk}(X_0,Y_0) & \{ \varphi( X_{s_1},Y_{s_1}) - \varphi( X_{s_1}',Y_{s_1}')\}] \\
 & \leqslant   ( 1 + \epsilon_1) \mathbb E[\1_{\rset^d \times \msy \setminus \msk}(X_0,Y_0)\{ V_1( X_{s_1}) + V_1( X_{s_1}')\}]\\
                                                             &  \leqslant  2 ( 1 + \epsilon_1) \parenthese{  \expe{\1_{\rset^d \times \msy \setminus \msk}(X_0,Y_0) V_1(X_0)} + A_2}\\
                                                             & \leq 2 ( 1 + \epsilon_1) \parenthese{ C \int_{U\geqslant l} \rme^{ U(x)/2}  \tpi_{k-1}(\rmd x)  + A_2} \\
%   \label{eq:second_bound_decomp_recuit}
   & \leq 2 ( 1 + \epsilon_1) \parenthese{ C \rme^{-(\beta_{k}-1)l/2} +A_2} \eqsp.
 \end{align*}
where we used for the penultimate inequality  that $(X_0,Y_0)$ is distributed according to $\tpi_{k-1}$,
Combining this result and  \eqref{eq:first_bound_decomp_recuit}  in \eqref{eq:decomp_recuit} and \eqref{eq:bound_rho_eps_k}, we get there exist $A_{6,2} \geq 0$ independent of $l$ and $A_{l,2} \geq 0$ satisfying 
\begin{equation*}
  %\label{eq:2}
  \rho_{\epsilon_{k}}( \tpi_{k-1} Q_{k},\tpi_{k-1} ) \leq A_{l,2}(\beta_{k}-\beta_{k-1}) + A_{6,2}   \rme^{-(\beta_{k}-1)l/2} \eqsp.
\end{equation*}
The proof is concluded combining this result and \eqref{eq:recuit_first_bound_main_lemma} in \eqref{eq:borne-en-recuit}. 
\end{proof}

%We can now state the main result of this section:
\begin{lemma}
  \label{lem:recuit-an}
Assume  \Cref{ass:recuit}. There exists $\theta >0$ such that if \Cref{ass:recuit-beta} holds with  $D_1 \leq \theta^{-1}$,
then
 there exists $A_7 >0$ satisfying for all $t\geqslant t_0$,  $k\leqslant \bfn(t)$ and $(x,y) \in \rset^d\times \msy$,
$
u_{k} \leq A_7V_1(x,y) /k^{q_1}$
where $u_{k}$ is given in \eqref{eq:def_an}  and  $q_1 = (1/2) (1 - \theta D_1)$.
\end{lemma}



\begin{proof}
  Let $l \geq 1$, $t \geq t_0$ and $k \in \{1,\ldots \bfn(t)\}$.
  In the proof, $C$ stands for a constant which may change from line to line but does not depend on $k$, $l$ and $\beta$.  Denoting $d_0=0$ and $d_{k} = \kappa_{k}  d_{k-1} + e_{k} $, \eqref{eq:recuit-an-en} reads
\begin{equation*}
u_{k} - d_{k}  \leqslant  \kappa_{k} ( u_{k-1} - d_{k-1})
\end{equation*}
and yields
\begin{equation}
  \label{eq:bound_a_k}
u_{k}  \leqslant    u_0 \prod_{j=1}^k \kappa_j +   \sum_{i=1}^k \defEns{ e_i \prod_{j=i}^{k-1} \kappa_j }\eqsp,
\end{equation}
with the convention that $\prod_{j=k}^{k-1} \kappa_j = 1$. From \Cref{lem:recuit-en} applied with $l=1/D_2$, and bounding
\[\beta_{k} - \beta_{k-1} \ \leqslant \ \frac{D_1\lceil s_1/s_0\rceil }{t - (\bfn(t)-k+1)s_1}\]
for $k$ large enough, we get
\begin{equation}
  \label{eq:bound_ek}
  e_{k} \leqslant C/\sqrt{k} \eqsp
\end{equation}
Let  $\theta = 2A_5 s_1$,  so that, by definition of $\kappa_k$ given in \Cref{lem:convergence} the condition $\beta$,  and using $1-s \leq \rme^{-s}$, we have 
\[\kappa_{k}\ \leqslant \ 1 - \parenthese{ \frac{\chi}2 \wedge \frac{1-\gamma}{4}}\exp ( - \theta \beta_{k}/2 ) \ \leqslant \ \exp( - C n^{-\theta D_1/2}) \]
 Hence, for $i\in\{1,\ldots,k\}$,
 \begin{equation*}
%   \label{eq:5}
   \prod_{j=i}^k \kappa_j \ \leqslant \exp\parenthese{ -C \sum_{j=i}^n j^{-\theta D_1/2}} \leqslant \exp\parenthese{ -(C/q)\{  (n+1)^{q} - i^{q}\}} \eqsp,
 \end{equation*}
with $q= 1 - \theta D_1/2 \in\ooint{1/2,1}$ by assumption. Thus, combining this result and \eqref{eq:bound_ek} in \eqref{eq:bound_a_k}, we get
%\begin{equation*}
% \prod_{j=i}^n \kappa_j %\leqslant % \exp( {-\frac{\bar \chi}{2}\sum_{j=i}^n \rme^{-\theta \beta_{j}}})\\ 
%  \leqslant  \exp( {-\frac{\bar \chi}{2} \rme^{-\theta \beta_{0}}\sum_{j=i}^n (j+1)^{-\theta D_1}}) \\
%   \leqslant  \exp( {-c_4( (n+1)^{q} - (i+1)^{q }) })
%\end{equation*}
%
%First, note that $\epsilon_{k}$ decays with $n$, so that $\|\cdot\|_1 \leqslant \rho_{\epsilon_k}\leqslant \rho_{k-1}$. Denoting $n=\lfloor t/t_1\rfloor$, since $\mu_{\beta_t} = \mu_{k}$ is invariant for $P_s^{\beta_{k}}$, then for all $s\geqslant 0$,
%\begin{eqnarray}\label{EqRecuitDemo}
%\|\nu P_{0,t}^{(\beta)} - \mu_{\beta_t}\|_1  \leqslant  \|\nu P_{0,n t_1}^{(\beta)} - \mu_{k}\|_1\notag\\
% \leqslant  \rho_{k-1}( \nu P_{0,n t_1}^{(\beta)} , \mu_{k-1} ) + \rho_{\epsilon_k}( \mu_{k} , \mu_{k-1} )
%\end{eqnarray}
%(with the convention $\mu_{-1} = \mu_0$ and $\rho_{-1}=\rho_0$). For $n\in\mathbb N$, set
%\begin{equation*}
%a_{k}  =  \rho_{k-1}( \nu P_{0,n t_1}^{(\beta)} , \mu_{k-1} )\\
% =  \rho_{k-1}( \nu Q_0\cdots Q_{k-1},\mu_{k-1} Q_{k-1})\\
% \leqslant  \kappa_{k-1} ( a_{k-1} + e_{k-1}) 
%\end{equation*}
%(with the convention $\kappa_{-1}=1$, $a_{-1}=a_0$ and $e_{-1}=0$). Let $d_0=0$ and $d_{n+1} = \kappa_{k}( d_{k} + e_{k})$ for all $n\geqslant 0$, this reads
%\begin{equation*}
%a_{n+1} - d_{n+1}  \leqslant  \kappa_{k} ( a_{k} - d_{k}) 
%\end{equation*}
%and thus, 
%\begin{equation*}
%a_{n+1}  \leqslant    a_0 \prod_{j=0}^n \kappa_j +   \sum_{i=1}^n ( e_i \prod_{j=i}^n \kappa_j ).
%\end{equation*}
%Now, we use that
%\[ \beta_0 + D_2 ( \ln(n+2) - \ln 2) \ < \ \beta_{k} \ < \ \beta_0 + D_1 \ln (n+1). \]
% In particular, in Lemma \ref{LemRecuit2}, we chose $l= l_0\vee  ( 16/D_2)$, which proves there exists some $c_3>0$ such that
%\begin{equation*}
%e_{k}  \leqslant  \frac{c_3}{(n+1)}
%\end{equation*}
%
%
%
%Using that that $(i+1)^{q} \leqslant i^{q}+1$, we end up with
\begin{equation*}
u_{k}  \leqslant    u_0 \rme^{-(C/q) (n^{q}-1)}+  C ( k^{-1/2} + I(k))  
\end{equation*}
with
\begin{align*}
I(k) & =  \rme^{-(C/q) k^q }\int_1^{k} \frac1{\sqrt{s}} \rme^{(C/q) s^q}\rmd s \\
& = \frac1{C}\parenthese{ \frac{1}{k^{q-\frac12}} - \rme^{-(C/q) (k^q -1)} }+ \frac{\rme^{-(C/q) k^q }}{C}( q - 1/2) \int_1^k s^{q-\frac32} \rme^{(C/q) s^q}\rmd s\\
&\leqslant   \frac{1}{C k^{q-\frac12}}  + \frac{\rme^{-(C/q) k^q }}{C} \int_1^{k_0} s^{q-\frac32} \rme^{(C/q) s^q}\rmd s + \frac{I(k)}{C k_0^{1-q}}
%& =  \frac{1}{q n^q} - \frac1{q}{\rme^{-n^q}} + \rme^{-n^q} \int_1^n \frac{1}{s^{1+q}} \rme^{s^q} \dd s\\
%& \leqslant  \frac{1}{q n^q}  +  \rme^{-n^q} \int_1^2 \frac{1}{s^{1+q}} \rme^{s^q} \dd s + \frac1{2^q} I,
\end{align*}
for all $k_0\geqslant 1$. In particular, for $k_0\geqslant (2/C)^{1/(1-q)}$, this means $I(k) \leqslant Ck^{1/2-q}$.

Finally, from the first part  \Cref{corollary-recuit}, $u_0 \leqslant C  V_1(x,y)$.
\end{proof}
% so that $I\leqslant c_5 n^{-q}$ for some $c_5>0$. As a consequence, \eqref{EqRecuitDemo} implies that
% \begin{equation*}
%\|\nu P_{0,t}^{(\beta)} - \mu_{\beta_t}\|_1 & \leqslant & \frac{c_6}{t^q}
%\end{equation*}
%for some $c_6>0$.
%
%In particular, if $\widetilde X^{(\beta)}_t$ is a random variable with law $\mu_{\beta_t}$ and $\mathsf A$ is a measurable set of $\R^d$, then 
%\begin{equation*}
%\mathbb P ( X^{(\beta)}_t \in \mathsf A ) & \leqslant & \mathbb P ( \widetilde X^{(\beta)}_t \in \mathsf A )  + \frac{c_6}{2 t^q}. 
%\end{equation*}
%Let $\mathsf A_0 = \{x\in\R^d,\   U(x) < \eta-\eta'\}$ and  $\mathsf A_1 = \{x\in\R^d,\ \eta < U(x) < \eta + \frac{\rho}{4}|x|^2\}$, which are a compact sets, and $\mathsf A_2 = \{x\in\R^d,\   U(x) > \eta+ \frac{\rho}{4}|x|^2\}$. Then
%\begin{equation*}
%\mathbb P ( \widetilde X^{(\beta)}_t \in \mathsf A )  & \leqslant & \frac{\rme^{-\beta_t \eta}( vol(\mathsf A_1) + \int_{\mathsf A_2} \rme^{-\frac{\rho}{4}|x|^2 }\dd x)}{\rme^{-\beta_t( \eta'-\eta)} vol(\mathsf A_0)}\\
%& \leqslant & \frac{c_7}{t^{D_2 \eta'}}
%\end{equation*}
%for some $c_7>0$, which concludes.


\begin{proof}[Proof of  \Cref{thm:ThmRecuit}]
Let $t>t_0$, $n= \bfn(t)$, $\eta>\eta'>0$.   In the proof, $C$ stands for a constant which may change from line to line but does not depend on $n$, $\eta,\eta',t$ and $\beta$. First,
\begin{equation*}
\mathbb P ( U(X^{(\beta)}_t) > \eta + \min U )   \leqslant  \int_{\{U\geqslant \eta\}} \tpi_{k}(\rmd x,\rmd y) + (1/2) \tvnorm{ P_{0,t}((x,y),\cdot) - \tpi_{k}}\eqsp.
\end{equation*}
  Similarly to \eqref{eq:recuit-masse},
\begin{equation*}
\int_{\{U\geqslant \eta\}} \tpi_{k}(\rmd x,\rmd y)    \leqslant   C \rme^{-\beta_{k} \eta'} \ \leqslant \  C t^{-D_2\eta'}\eqsp.
\end{equation*}
We conclude, with \Cref{lem:recuit-an} and the first part of \Cref{corollary-recuit}, by
\begin{equation*}
\tvnorm{\nu P_{0,t} - \tpi_{k}}  \leqslant   u_{k} \ \leqslant C V_1(x,y) /t^q \eqsp.
\end{equation*}
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_supplement"
%%% End:

